Graph Machine Learning in the Era of Large Language Models (LLMs)

Graphs play an important role in representing complex relationships in various domains like social networks, knowledge graphs, and molecular discovery. With the advent of deep learning, Graph Neural Networks (GNNs) have emerged as a cornerstone in Graph Machine Learning (Graph ML), facilitating the representation and processing of graphs. Recently, LLMs have demonstrated unprecedented capabilities in language tasks and are widely adopted in a variety of applications such as computer vision and recommender systems. This remarkable success has also attracted interest in applying LLMs to the graph domain. Increasing efforts have been made to explore the potential of LLMs in advancing Graph ML's generalization, transferability, and few-shot learning ability. Meanwhile, graphs, especially knowledge graphs, are rich in reliable factual knowledge, which can be utilized to enhance the reasoning capabilities of LLMs and potentially alleviate their limitations such as hallucinations and the lack of explainability. Given the rapid progress of this research direction, a systematic review summarizing the latest advancements for Graph ML in the era of LLMs is necessary to provide an in-depth understanding to researchers and practitioners. Therefore, in this survey, we first review the recent developments in Graph ML. We then explore how LLMs can be utilized to enhance the quality of graph features, alleviate the reliance on labeled data, and address challenges such as graph Heterophily and out-of-distribution (OOD) generalization. Afterward, we delve into how graphs can enhance LLMs, highlighting their abilities to enhance LLM pre-training and inference. Furthermore, we investigate various applications and discuss the potential future directions in this promising field.

==> Figs/RefTree.tex <==
\definecolor{mycolor}{RGB}{215, 245, 200}

\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzset{
leaf/.style={
my-box,
minimum height=1.5em,
fill=mycolor, % Change the RGB values to the desired values
text=black,
align=left,
font=\footnotesize,
inner xsep=2pt,
inner ysep=4pt,
line width=0.8pt
}
}
\begin{figure*}[t!]
    \centering
    \begin{adjustbox}{width=0.95\textwidth}
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                text centered,
                minimum width=5em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=10em,font=\normalsize,}{},
            where level=2{text width=12em,font=\normalsize,}{},
            where level=3{text width=12em,font=\normalsize,}{},
            where level=4{text width=10em,font=\normalsize,}{},
            where level=5{text width=7em,font=\normalsize,}{},
            where level=6{text
            width=7em,font=\normalsize,}{},
            [Graph Machine Learning\\in the Era of LLMs
                [Background (Sec.\ref{sec:related work})
                    [Graph Machine Learnig\\(Sec.\ref{sec:graph ml})
                        [LINE~\cite{tang2015line}{,} DeepWalk~\cite{perozzi2014deepwalk}{,} Node2Vec~\cite{grover2016node2vec}{,} GCN~\cite{kipf2016semi}{,} GraphSAGE~\cite{hamilton2017inductive}{,} GAT~\cite{velivckovic2017graph}{,} GraphFormer~\cite{yang2021graphformers}, leaf, text width=36em]
                    ]
                    [LLMs (Sec.\ref{sec:llms})
                        [GPT~\cite{radford2018improving}{, }Bert ~\cite{devlin2018bert}{, } T5~\cite{raffel2020exploring}{, } 
                        GPT-3~\cite{brown2020language}{, }LaMDA~\cite{thoppilan2022lamda}{, } PaLM~\cite{chowdhery2022palm}{, } Vicuna~\cite{chiang2023vicuna}, leaf, text width=30em]
                    ]
                ]
                [Deep Learning\\on Graphs (Sec.\ref{sec:graph foundation model})
                    [Backbone Architecture\\(Sec.\ref{sec:backbone})
                        [Neighborhood\\Aggregation-based Model\\(Sec.\ref{sec:neighborhood aggregation})
                            [GCN~\cite{kipf2016semi}{, } CSSL~\cite{zeng2021contrastive}{,} PRODIGY~\cite{huang2023prodigy}{,} GraphSAGE~\cite{hamilton2017inductive}{,}\\PinSage~\cite{ying2018graph}{,} GAT~\cite{velivckovic2017graph}{,} GIN~\cite{xu2018powerful}, leaf, text width=20em]
                        ]
                        [Graph Transformer-based\\Model (Sec.\ref{sec:graph transformer})
                        [Heterformer~\cite{jin2023heterformer}{,}  Edgeformers~\cite{jin2023edgeformers}{,} Graph-Bert~\cite{zhang2020graph}{,}\\GROVER~\cite{rong2020self}
                        GraphGPT~\cite{zhao2023graphgpt}, leaf, text width=20em]
                        ]
                    ]
                    [Self-Supervised Learning\\on Graphs(Sec.\ref{sec:ssl})
                        [Graph Pretext Tasks\\(Sec.\ref{sec:Graph Pretext Tasks})
                        [GRACE~\cite{zhu2020deep}{, } CSSL~\cite{zeng2021contrastive}{,} GCC~\cite{qiu2020gcc}{,} DGI~\cite{velivckovic2018deep}{,} GraphCL~\cite{you2020graph}\\
                        GraphMAE~\cite{hou2022graphmae}{,} Graph-Bert~\cite{zhang2020graph}{,} GROVER~\cite{rong2020self}{,} \citet{hu2019pre}, leaf, text width=23em]
                        ] 
                        [Downstream Adaptation\\(Sec.\ref{sec:Downstream Adaptation})
                            [DGI~\cite{velivckovic2018deep}{,} \citet{zhang2020graph,you2020graph,zeng2021contrastive}{,}\\\citet{li2023adaptergnn,gui2023g,you2020graph}{,} AdapterGNN~\cite{li2023adaptergnn}{,}\\ GPPT~\cite{sun2022gppt}{,} GraphPrompt~\cite{liu2023graphprompt}{,} Prog~\cite{sun2023all} , leaf, text width=23em]
                        ]
                    ]
                ]
                [LLMs for Graph Models\\ (Sec.\ref{sec:LLM-enhanced Graph})
                    [Enhancing Feature Quality \\(Sec.\ref{sec:enhance feature})
                        [Enhancing Feature\\Representation (Sec.\ref{sec:enhance rep})
                        [Patton \cite{jin2023patton}{, }METERN \cite{jin2023learning}{, }\citet{chen2023exploring}{, }LKPNR \cite{hao2023lkpnr}{, }\\SimTeG \cite{duan2023simteg}, leaf, text width=20em]
                        ]
                        [Generating Augmented\\Information (Sec.\ref{sec:Generating Augmented Information})
                        [TAPE \cite{he2023harnessing}{, }KEA \cite{chen2023exploring}{, }
                        LLM4Mol \cite{qian2023can}{, }GPT-MolBERTa \cite{balaji2023gptmolberta}{, }\\LLM-Rec \cite{lyu2023llmrec}{, }LLMRec \cite{weillmrec}{, }ENG~\cite{yu2023empower}{, }\citet{sun2023large}, leaf, text width=22em]
                        ]
                        [Aligning Feature Space\\(Sec.\ref{sec:Aligning Feature Space})
                        [TouchUp-G \cite{zhu2023touchup}{, }OFA \cite{liu2023one}, leaf, text width=10em]
                        ]
                    ]
                    [Solving Vanilla GNN\\Training Limitations (Sec.\ref{sec:Solving Vanilla GNN Training Limitations})
                        [Ignoring Structural\\Information
                            (Sec.\ref{sec:Ignoring Structural Information})
                            [\citet{hu2023text}, leaf, text width=5em]
                        ]
                        [Implicit Structural\\Information (Sec.\ref{sec:Implicit Structural Information})
                            [\citet{hu2023text,huang2023can}{, }NLGraph \cite{wang2023can}{, }\\
                            \citet{ye2023natural}{, }GraphEdit \cite{guo2024graphedit}{, }GPT4Graph~\cite{guo2023gpt4graph}{, }\\GraphText~\cite{zhao2023graphtext}, leaf, text width=18em]
                        ]
                        [Explicit Structural\\Information (Sec.\ref{sec:Explicit Structural Information})
                            [GIT-Mol~\cite{liu2023gitmol}{, }KoPA~\cite{zhang2023making}{, }
                            GIMLET~\cite{zhao2023gimlet}{, }\\GraphToken~\cite{perozzi2024let}{, }ProteinChat~\cite{guo2023proteinchat}{, }DrugChat~\cite{liang2023drugchat}{, }\\GraphLLM~\cite{chai2023graphllm}{, }BioMedGPT~\cite{luo2023biomedgpt}, leaf, text width=18em]
                        ]
                    ]
                    [Heterophily and\\Generalization (Sec.\ref{sec:Heterophily and Generalization})
                            [GraphText~\cite{zhao2023graphtext}{, }Chen et al.~\cite{chen2023exploring}{, }OpenGraph~\cite{xia2024opengraph}, leaf, text width=18em]
                    ]
                    [Improving GNN\\Trustworthiness (Sec.\ref{sec:Improving GNN Trustworthiness})
                        [Robustness
                            (Sec.\ref{sec:Robustness})
                            [\citet{guo2024learning}{,} LLM4RGNN~\cite{zhang2024can}, leaf, text width=12em]
                        ]
                        [Privacy (Sec.\ref{sec:Privacy})
                            [~\citet{guan2024large}, leaf, text width=7em]
                        ]
                        [Explainability (Sec.\ref{sec:Explainability})
                            [\citet{zhang2024llmexplainer}{, } LLM-GCE~\cite{he2024explaining}, leaf, text width=12em]
                        ]
                    ]
                ]
                [Graphs for LLMs (Sec.\ref{sec:Graph-enhanced LLMs})
                    [KG-enhanced (L)LM\\Pre-training (Sec.\ref{sec:KG-enhanced (L)LM Pre-training})
                        [Modifying Input Data\\(Sec.\ref{sec:Modifying Input Data})
                            [\citet{moiseev2022skill} {, }E-BERT~\cite{poerner2019bert}{, }KALM~\cite{rosset2020knowledge}{, } K-BERT~\cite{liu2020kbert}, leaf, text width=22em]
                            ]
                        [Modifying Model Structures\\ (Sec.\ref{sec:Modifying Model Structures})
                            [ERNIE~\cite{zhang2019ernie}{, }CokeBERT~\cite{su2021cokebert}{, }
                            KLMO~\cite{he2021klmo}{, }K-Adapter~\cite{wang2021kadapter}{, }\\KALA~\cite{kang2022kala}{, }DAKI~\cite{lu2021parameter}, leaf, text width=22em]
                            ]
                        [Modifying Pre-training Tasks\\ (Sec.\ref{sec:Modifying Pre-training Tasks})
                            [ERNIE~\cite{zhang2019ernie}{, }LUKE~\cite{yamada2020luke}{, }
                            KILM~\cite{xu2023kilm}{, }GLM~\cite{shen2020exploiting}{, }JAKET~\cite{yu2022jaket}{, }\\Dragon~\cite{yasunaga2022deep}{,}ERICA~\cite{qin2020erica}, leaf, text width=22em]
                            ]
                    ]
                    [KG-enhanced LLM Inference\\(Sec.\ref{sec:KG-enhanced LLM Inference})
                            [Enhancing by In-Context\\Learning~(\ref{sec:icl})
                                [RoG~\cite{luo2023reasoning}{, }Knowledge Solver~\cite{feng2023knowledge}{, }Keqing~\cite{wang2023keqing}{, }\\Mindmap~\cite{wen2023mindmapa}{, }KGR~\cite{guan2023mitigating}{, }ChatGraph~\cite{shi2023chatgraph}{, }\\XplainLLM~\cite{chen2023xplainllm}
                                        , leaf, text width=18em]
                            ] 
                            [Enhancing by Fine-tuning\\(\ref{sec:finetuning})
                                [~\citet{tian2024kg}{, } KG-Agent~\cite{jiang2024kg}{, } InfuserKI~\cite{wang2024infuserki}
                                        , leaf, text width=18em] 
                            ]
                    ]
                ]
                [Applications (Sec.\ref{sec:application})
                    [Recommender Systems\\(Sec.\ref{sec:Recommender Systems})
                            [\citet{liu2023chatgpt}{, } TallRec~\cite{bao2023tallrec}{, } KAR~\cite{xi2023towards} {,} LLM-Rec~\cite{lyu2023llmrec}{,}\\RLMRec~\cite{ren2023representation}{,} LLMRec~\cite{weillmrec}{,}~\citet{wu2022disentangled}{,} OFA~\cite{tang2023one}{,}\\UP5~\cite{hua2023up5}{,} \citet{huang2024foundation}, leaf, text width=20em]
                    ]
                    [Knowledge Graphs (Sec.\ref{sec:Knowledge Graphs})[
                            KG-Bench~\cite{meyer2023developing}{,} KG-LLM~\cite{yao2023exploring}{,} KG-GPT~\cite{kim2023kggpt}{,}\\ChatKBQA~\cite{luo2023chatkbqa}{,} \citet{wu2023retrieverewriteanswer}{,} Ultra~\cite{galkin2023towards}, leaf, text width=18em]
                    ]
                    [AI for Science (Sec.\ref{sec:AI for Science})              [
                    MolReGPT~\cite{li2023empowering}{,} GPT-MolBERTa~\cite{balaji2023gptmolberta}{,} ReLM~\cite{shi2023relm}{,}\\ChemCrow~\cite{bran2023chemcrow}{,} InstructMol~\cite{cao2023instructmol}{,} ChemDFM~\cite{zhao2024chemdfm}
                    , leaf, text width=18em]
                    ]
                    [Robot Task Planning (Sec.\ref{sec:Robot Task Planning})[
                    ~\citet{chalvatzaki2023learning}{,} SayPlan~\cite{rana2023sayplan}{,}\\\citet{zhen2023robot}{,} GRID~\cite{ni2023grid}
                    , leaf, text width=18em]
                    ]
                ]
                [Future Directions (Sec.\ref{sec:future_work}) 
                    [Retrieval-Augmented\\Generation with Graphs\\(Sec.\ref{sec:GraphRAG})
                    [G-retriever~\cite{he2024g}, leaf, text width=5em]
                    ]
                    [Generalization and\\Transferability (Sec.\ref{sec:Generalization and Transferability})
                    [OFA~\cite{liu2023one}, leaf, text width=5em]
                    ]
                    [Trustworthiness (Sec.\ref{sec:future-Trustworthiness})
                        [Robustness\&Safety (Sec.\ref{sec:Robustness-Safety})
                            % [DeepST \cite{zhang2016dnn}{, }\citet{bai2019spatio}{, }ROD-Revenue \cite{guo2019rod}, leaf, text width=20em]
                            ]
                        [Explainability (Sec.\ref{sec:future-Explainability})
                            [P5~\cite{geng2022recommendation}, leaf, text width=3em]
                            ]
                        [Fairness (Sec.\ref{sec:Fairness})
                            [\citet{webster2020measuring}{,} Auto-Debias~\cite{guo2022auto}{,} Mabel~\cite{he2022mabel}{,} FairNeg~\cite{chen2023fairly}, leaf, text width=22em]
                        ]
                        [Privacy (Sec.\ref{sec:future-Privacy})
                            [PART~\cite{li2023privacy}, leaf, text width=5em]
                            ]
                    ]
                    [Efficiency (Sec.\ref{sec:future-Efficiency})[LoRA~\cite{hu2021lora}{,} QLoRA~\cite{dettmers2023qlora}{,} LLM-Pruner~\cite{ma2023llm}{,} Sheared llama~\cite{xia2023sheared} , leaf, text width=22em]
                    ]
                    [Multi-modal Graph Learning\\(Sec.\ref{sec:Multi-modal Graph Learning})[TOUCHUP-G~\cite{zhu2023touchup}, leaf, text width=8em]
                    ]
                ]
            ]
        \end{forest}
    \end{adjustbox}
        \vspace{-4mm}
    \caption{Summary of relevant methods for each section in our survey.}
    \label{fig:ref tree}
\end{figure*}

==> Figs/summary-of-enhancer.tex <==
\begin{figure}[t]
\centering
\scriptsize
\begin{tikzpicture}
[node distance=0.5cm,
  level 1/.style={sibling distance=30mm},
  % level 1/.style={sibling distance=30mm, every node/.style={fill=red!30!white}},
  % level 2/.style={every node/.style={fill=green!30}},
  % level 3/.style={every node/.style={fill=blue!30}},
  edge from parent/.style={->,draw},
  >=latex][t]
\node[root] {LLM as Enhancer}
% The first level, as children of the initial tree
  child {node [level 2] (c1) {Feature-Level}}
  child {node[level 2] (c2) {Text-Level}}
  child {node[level 2] (c3) {Data-Level}};

% The second level, relatively positioned nodes
\begin{scope}[every node/.style={level 3}]
\node [below of = c1] (c10) {\textbf{Text Embedding}};
\node [below of = c10, xshift=5pt ] (c11)
{Chen et al.~\cite{chen2023exploring}};
\node [below of = c11 ] (p11)
{SimTeG~\cite{duan2023simteg}};
\node [below of = p11 ] (p12)
{LKPNR~\cite{hao2023lkpnr}};
\node [below of = p12 ] (p13)
{GRID~\cite{ni2023grid}};

\node [below of = c2] (c20) {\textbf{Labels}};
\node [below of = c20 , xshift=5pt] (c21)
{TAPE~\cite{he2023harnessing}};
\node [below of = c21, xshift=-5pt] (c22) {\textbf{Descriptions}};
\node [below of = c22, xshift=5pt ] (p28)
{KEA~\cite{chen2023exploring}};
\node [below of = p28 ] (p29)
{RLMRec~\cite{ren2023representation}};
\node [below of = p29 ] (p30)
{LLMRec~\cite{weillmrec}};
\node [below of = p30 ] (p31)
{LLM-Rec~\cite{lyu2023llmrec}};
\node [below of = p31 ] (p32)
{GPT-MolBERTa~\cite{balaji2023gptmolberta}};
\node [below of = p32 ] (p33)
{LLM4Mo~\cite{qian2023can}};


\node [below of = c3 ] (c31) {\textbf{Nodes}};
\node [below of = c31 , xshift=5pt] (c31)
{LLMRec~\cite{weillmrec}};
\node [below of = c31, xshift=-5pt] (p311) {\textbf{Relations}};
\node [below of = p311, xshift=5pt  ] (p31)
{ENG~\cite{yu2023empower}};
\end{scope}


\end{tikzpicture}
\caption{A summary of LLM-as-Enhancer research, categorized by \emph{feature-level},\emph{text-level}, and \emph{data-level}. 
To be specific, \emph{feature-level} enhancement methods typically use LLM as text encoder to get text embedding, \emph{text-level} enhancement leverages the reasoning capabilities of LLMs to generate semantically enriched text such as labels and explanations, and \emph{data-level} enhancement involves utilizing LLMs for data augmentation from the perspectives of nodes and relations.
} 
\label{fig:summary-of-enhancer}
\end{figure}



==> Figs/summary-of-predictor.tex <==
\begin{figure}[t]
\centering
\scriptsize
\begin{tikzpicture}
[node distance=0.5cm,
  level 1/.style={sibling distance=30mm},
  edge from parent/.style={->,draw},
  >=latex][t]
\node[root] {LLM as Predictor}
% The first level, as children of the initial tree
  child {node[level 2] (c1) {Graph-to-Text Method}}
  child {node[level 2] (c2) {Graph-Text Fusion Method}};

% The second level, relatively positioned nodes
\begin{scope}[every node/.style={level 3}]
\node [below of = c1 ] (c11)
{GPT4Graph~\cite{guo2023gpt4graph}};
\node [below of = c11 ] (p11)
{GraphText~\cite{zhao2023graphtext}};
\node [below of = p11 ] (p12)
{NLGraph~\cite{wang2023can}};
\node [below of = p12 ] (p13)
{InstructGLM~\cite{ye2023natural}};
\node [below of = p13 ] (p14)
{LLMtoGraph~\cite{liu2023evaluating}};
\node [below of = p14 ] (p15)
{LLM-Prop~\cite{rubungo2023llmprop}};
\node [below of = p15 ] (p16)
{GLRec~\cite{wu2023exploring}};
\node [below of = p16 ] (p17)
{ReLM~\cite{shi2023relm}};
\node [below of = p17 ] (p18)
{Chen et al.~\cite{chen2023exploring}};
\node [below of = p18 ] (p19)
{Hu et al.~\cite{hu2023text}};
\node [below of = p19 ] (p20)
{Huang et al.~\cite{huang2023can}};
\node [below of = p20 ] (p21)
{Fatemi et al.~\cite{fatemi2023talk}};
\node [below of = p21 ] (p22)
{MolReGPT~\cite{li2023empowering}};
            
\node [below of = c2 ] (c21)
{GraphGPT~\cite{tang2023graphgpt}};
\node [below of = c21 ] (p21)
{ GraphLLM~\cite{chai2023graphllm}};
\node [below of = p21 ] (p22)
{GNP~\cite{tian2023graph}};
\node [below of = p22 ] (p23)
{KoPA~\cite{zhang2023making}};
\node [below of = p23 ] (p24)
{GIT-Mol~\cite{liu2023gitmol}};
\node [below of = p24 ] (p25)
{DrugChat~\cite{liang2023drugchat}};
\node [below of = p25 ] (p26)
{BioMedGPT~\cite{luo2023biomedgpt}};
\node [below of = p26 ] (p27)
{ProteinChat~\cite{guo2023proteinchat}};
\node [below of = p27 ] (p28)
{DGTL~\cite{qin2023disentangled}};


\end{scope}

\end{tikzpicture}
\caption{A summary of LLM-as-Predictor research, categorized by Graph-to-Text Method and Graph-Text Fusion Method. }
\label{fig:summary-of-predictor}
\end{figure}

\begin{figure*}[tb]
 \centering
\includegraphics[width=\linewidth]{Figs/LLM as Predictor4.pdf}
\caption{The illustration of LLMs as Predictors approaches. \textbf{Graph-to-Text-based} methods describe nodes and graph structure information in natural language and combine task-specific instructions to form a textual prompt, which is then input into the LLM to generate prediction results. \textbf{Graph-Text-Fusion-based} methods use GNNs and LLMs to encode graph and instruction information separately. Fusion layers are added to integrate modalities, and the fused vector is input into the LLM for prediction.}
\label{fig:llm as predictor}
\end{figure*}

==> Tables/experiment-summary.tex <==
\begin{table*}[htbp]
  \centering
  \caption{A summary of experiment results of LLM-enhanced graph learning methods on node classification datasets. $\star$ represents Instruction Tuning.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccccc}
    \toprule
    \multicolumn{1}{c}{Role} & \multicolumn{1}{c}{Subcategory} & Method & LLM & CORA & PUBMED & OGBN-ARXIV & OGBN-PRODUCTS & CiteSeer \\
    \midrule
    \multirow{5}[6]{*}{\rotatebox{90}{As Enhancer}} & \multirow{2}[0]{*}{Feature-level} & Chen et al.~\cite{chen2023exploring} & LLaMA-7B & 66.80 ± 2.20 & 73.53 ± 0.06 & - & - & - \\
      &   & SimTeG~\cite{duan2023simteg} & e5-large, etc. & - & - & 78.03 ± 0.07 & - & - \\
     \cmidrule{2-9}  & \multirow{2}[2]{*}{Text-level} & KEA~\cite{chen2023exploring} & ChatGPT, e5-large & 85.02 ± 0.40 & 83.30 ± 1.75 & - & - & - \\
      &   & TAPE~\cite{he2023harnessing} & ChatGPT, DeBERTa & 92.90 ± 3.07 & 96.18 ± 0.53 & 77.50 ± 0.12 & 82.34 ± 0.36 & - \\
      \cmidrule{2-9}   & Data-level & ENG~\cite{yu2023empower} & ChatGPT, MiniLM & 80.94 ± 1.55 & 80.54 ± 0.78 & 61.40 ± 1.06 & - & - \\
      \midrule
      
    \multirow{8}[4]{*}{\rotatebox{90}{As Predictor}} & \multirow{7}[0]{*}{Graph-to-Text} & Chen et al.~\cite{chen2023exploring} & ChatGPT & 67.75 ± 3.53 & 90.75 ± 5.30 & 51.75 ± 3.89 & 77.75 ± 1.06 & 66.50 ± 2.82 \\
      &   & GraphText~\cite{zhao2023graphtext} & LLaMA-7B$\star$ & 87.11 & - & - & - & 74.77 \\
      &   & GraphText~\cite{zhao2023graphtext} & ChatGPT & 67.77 & - & - & - & 68.98 \\
          &   & InstructGLM~\cite{ye2023natural} & Flan-T5, LLaMA$\star$ & 90.77 ± 0.52 & 94.62 ± 0.13 & 75.70 ± 0.12 & - & - \\
      &   & Graph Agent~\cite{wang2023graph} & GPT-4 & 90.65 & 95.48 &   & - & - \\
      &   & Hu et al.~\cite{hu2023text} & ChatGPT & 65.6 & 83.3 & 67.3 &   & - \\
      &   & Huang et al.~\cite{huang2023can} & ChatGPT & 74.7 & 89.7 & 75.1 & 86.2 & - \\
      \cmidrule{2-9}   & Graph-Text Fusion & DGTL~\cite{qin2023disentangled} & Llama-2-13B-chat & 81.10 ± 0.20 & 87.10±1.31 & - & - & - \\
      \bottomrule
    \end{tabular}%
    }
    \label{tab:experiment summary}%
\end{table*}%

==> Tables/graph-enhanced_llm.tex <==
\begin{table*}[htbp]
  \centering
  \renewcommand{\arraystretch}{1.2}
  \caption{A summary of graph-enhanced LLM Research. \textbf{TC} in the Task column is the Text Classification task.}
  \label{tab:graph-enhanced LLM}%
   \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccccl}
    \toprule
    Role & \multicolumn{1}{c}{Method} & \multicolumn{1}{c}{Graph} & \multicolumn{1}{c}{GNN} & \multicolumn{1}{c}{LLM} & \makecell[c]{Fine\\Tuning} & \multicolumn{1}{c}{Domain}  & Task & Reasoning Basis & Link \\
    \midrule
    \multirow{3}[2]{*}{\rotatebox{90}{\makecell[c]{Alleviating\\Hallucination}}} & RANKING~\cite{khistegraph} & Document Graph & - & BART & \lightgreen{$\checkmark$} & - & QA & -  & - \\
      & KI~\cite{martino2023knowledge} & Knowledge Graph & - & \makecell[c]{text-davinci-003,\\bloom-560m} & \lightgreen{$\checkmark$} & E-commerce & QA & - & - \\
      & Li et al.~\cite{li2023verifiable} & Knowledge Graph & - & \makecell[c]{ChatGPT, GPT-4,\\LLaMA} & \lightgreen{$\checkmark$} & Biography & QA & Entity & -  \\
    \midrule
\multirow{6}[2]{*}{\rotatebox{90}{\makecell[c]{Improving\\Transparency\\}}} & ChatGraph\cite{shi2023chatgraph} & Text Graph & GCN & ChatGPT & \red{$\times$} & - & TC & Linear model & \href{https://github.com/sycny/ChatGraph}{link}  \\
      & XplainLLM~\cite{chen2023xplainllm} & Knowledge Graph & GAT & ChatGPT & \red{$\times$} & - & QA & LLM generated explanation  & \href{https://github.com/chen-zichen/XplainLLM_dataset.git}{link} \\
      & RoG~\cite{luo2023reasoning} & Knowledge Graph & - & LLaMA2-Chat-7B & \lightgreen{$\checkmark$} & Web & QA & Relation path & \href{https://github.com/RManLuo/reasoning-on-graphs}{link} \\
      & FE~\cite{saxena2023minimizing} & Knowledge Graph & - & ChatGPT, LLaMA-7B & \lightgreen{$\checkmark$} & Biomedical & QA  & Rationale & - \\
      & KGR~\cite{guan2023mitigating} & Knowledge Graph & - & \makecell[c]{text-davinci-003,\\ChatGPT, Vicuna-13B} & \red{$\times$} & - & QA & Claims & -  \\
      & MindMap~\cite{wen2023mindmapa} & Knowledge Graph & - & ChatGPT, GPT-4 & \red{$\times$} & Medical & QA & Evidence graph & \href{https://github.com/wylwilling/MindMap}{link}  \\
    \midrule
    \multirow{3}[2]{*}{\rotatebox{90}{\makecell[c]{Advancing\\Multi-step\\Reasoning}}} & GoT~\cite{besta2023graph} & - & - & ChatGPT, GPT-4 & \red{$\times$} & - & QA & - & \href{https://github.com/spcl/graph-of-thoughts}{link} \\
      & GoT~\cite{yao2023beyond} & - & GAT & T5 & \lightgreen{$\checkmark$} & - & QA & - & - \\
      & Rex-GoT\cite{zheng2023reverse} & - & - & Flan T5, ChatGPT & \red{$\times$} & - & QA & - & \href{https://github.com/ZhengL00/ReX-GoT}{link} \\
      & RGV~\cite{cao2023enhancing} & - & - & ChatGPT & \red{$\times$} & - & QA & - & - \\
    \bottomrule
    \end{tabular}%
    }
  
\end{table*}%

==> Tables/graph-to-text_methods.tex <==
\begin{table*}[t] 
  \centering
  \caption{Graph-to-Text Methods}
    \label{tab:graph2text}%
  \renewcommand\arraystretch{1.25}
    \resizebox{\linewidth}{!}{
  
    \begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}[4]{*}{Reference} & \multicolumn{3}{c}{Graph Encoding Methods} & \multirow{2}[4]{*}{\makecell[c]{Prompting Strategies}} & \multirow{2}[4]{*}{LLM Models} & \multicolumn{2}{c}{Tasks} & \multirow{2}[4]{*}{\makecell[c]{Instruction\\Tuning}} \\
\cmidrule{2-4}\cmidrule{7-8}    \multicolumn{1}{c}{} & \makecell[c]{Node\\Feature} & \makecell[c]{Neighbor\\Range} & \makecell[c]{Neighbor\\Structure} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \makecell[c]{Semantic\\Understanding} & \makecell[c]{Structure\\Understanding} & \multicolumn{1}{c}{} \\
    \midrule
    ~\cite{ye2023natural} & \lightgreen{$\checkmark$} & 1-hop, 2-hop, 3-hop & \lightgreen{$\checkmark$} & \textbackslash & \makecell[c]{Flan-T5, LLaMa-7b} & \lightgreen{$\checkmark$} & \red{$\times$} & \lightgreen{$\checkmark$}\\

    ~\cite{chen2023exploring} & \lightgreen{$\checkmark$} & 2-hop & \lightgreen{$\checkmark$} & zero-shot, few-shot, CoT & LLaMA & \lightgreen{$\checkmark$} & \red{$\times$} & \red{$\times$} \\

    ~\cite{guo2023gpt4graph} & \checkmark & 1-hop, 2-hop & \checkmark & \makecell[c]{zero-shot, few-shot, CoT,\\ role prompting,\\self-prompting} & text-davinci-003 & \checkmark & \checkmark & \red{$\times$}  \\

    ~\cite{zhao2023graphtext} & \lightgreen{$\checkmark$} & 2-hop & $\halfcheckmark$ & few-shot & LLaMA2-7b,ChatGPT & \lightgreen{$\checkmark$} & \red{$\times$} & \checkmark \\

    ~\cite{fatemi2023talk} & \red{$\times$} & all & \lightgreen{$\checkmark$} & \makecell[c]{zero-shot, few-shot, CoT,\\Bag prompting} & PaLM 62B,PALM 2 XXS & \red{$\times$} & \lightgreen{$\checkmark$} & \red{$\times$}\\

     ~\cite{wang2023can} & \red{$\times$} & all & \lightgreen{$\checkmark$} & \makecell[c]{zero-shot, few-shot, CoT,\\self-consistency,\\least-to-most, Bag prompting,\\Algorithmic Prompting} & 
    \makecell[c]{text-davinci-003, gpt-3.5-turbo,\\ coded-davinci-002, gpt-4} & \red{$\times$} & \lightgreen{$\checkmark$} & \red{$\times$}\\

    ~\cite{hu2023text} & \lightgreen{$\checkmark$} & 1-hop & $\halfcheckmark$ & zero-shot, few-shot & gpt-3.5-turbo-16k, gpt-4 & \lightgreen{$\checkmark$} & \red{$\times$} & \red{$\times$}\\

    ~\cite{huang2023can} & \lightgreen{$\checkmark$} & 1-hop, 2-hop & $\halfcheckmark$ & \makecell[c]{zero-shot, few-shot, CoT} & \makecell[c]{ChatGPT} & \lightgreen{$\checkmark$} & \red{$\times$} & \red{$\times$}\\
    \bottomrule
    \end{tabular}%
   }
\end{table*}%

==> Tables/llm-enhanced-graph-v1.tex <==
\begin{table*}[ht]
  \centering
  \caption{A summary of LLM-enhanced graph learning research. We present the GNN model, LLM model, predictor, domain, task, datasets, and project link. \textbf{FT} is Fine-tuning, refers to whether modifications are made to the parameters of the LLM model while \textbf{PR} is Prompting, involves inputting textual prompts to the LLM to obtain responses. In the context of \textbf{task}, "node" denotes node-level tasks such as node classification, "edge" signifies edge-level tasks like link prediction, "graph" represents graph-level tasks such as graph classification, and "structure" pertains to structure understanding tasks, such as node degree counting.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{rcccccccccc}
\cmidrule{1-11}    \multicolumn{1}{l}{Role} & Method & GNN Model & LLM Model & Predictor & FT & PR & Domain & Task & Datasets & Link \\
    \midrule
    \multicolumn{1}{c}{\multirow{3}[2]{*}{\rotatebox{90}{Annotator}}} & Graphologue~\cite{jiang2023graphologue} & - & GPT-4 & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & - & Information Extraction & 1 &\href{https://graphologue.app/}{link} \\ [1ex]
    & Karim et al.~\cite{karim2023large} & - & ChatGPT & - & \red{$\times$} & \lightgreen{$\checkmark$} & Bioinformatics & Information Extraction &- & - \\ [1ex]
    & LLM-GNN~\cite{chen2023labelfree} & GCN, SAGE & ChatGPT & GNN & \red{$\times$} & \lightgreen{$\checkmark$} & Citation, E-commerce & Node & 6& \href{https://github.com/CurryTang/LLMGNN}{link} \\ [1ex] 
    
    \midrule
    \multicolumn{1}{c}{\multirow{6}{*}[-8ex]{\rotatebox[origin=c]{90}{Enhancer}}} 
    
    & Chen et al.~\cite{chen2023exploring} & \makecell[c]{GCN, GAT, MLP,\\SAGE, etc.} & ChatGPT, LLaMA & GNN & \red{$\times$} & \lightgreen{$\checkmark$} & Citation, E-commerce & Node &5 & \href{https://github.com/CurryTang/Graph-LLM}{link} \\
      & SimTeG~\cite{duan2023simteg} & \makecell[c]{SAGE, MLP, etc.} & \makecell[c]{all- MiniLM-L6-v2, etc.} & GNN & \lightgreen{$\checkmark$} & \red{$\times$} & Citation, E-commerce & Node, Edge &3 & \href{https://github.com/vermouthdky/SimTeG}{link} \\
      & TAPE~\cite{he2023harnessing} & \makecell[c]{GCN, SAGE,MLP\\RevGAT} & ChatGPT, LLaMA2 & GNN & \red{$\times$} & \lightgreen{$\checkmark$} & Citation, E-commerce & Node &5& \href{https://github.com/XiaoxinHe/TAPE}{link} \\
      & RLMRec~\cite{ren2023representation} & LightGCN & ChatGPT  & GNN & \red{$\times$} & \lightgreen{$\checkmark$} & Recommendation & Recommendatoon &3& \href{https://github.com/HKUDS/RLMRec}{link} \\
      & LLMRec~\cite{weillmrec} & LightGCN & \makecell[c]{ChatGPT,\\gpt-3.5-turbo-16k} & GNN & \red{$\times$} & \lightgreen{$\checkmark$} & Recommendation & Recommendatoon & 2 & \href{https://github.com/HKUDS/LLMRec.git}{link} \\
      & LLM-Rec~\cite{lyu2023llmrec} & - & text-davinci-003 & MLP & \lightgreen{$\checkmark$} & \red{$\times$} & Recommendation & Recommendation&2 & - \\
      & LKPNR~\cite{hao2023lkpnr} & wiki KG & \makecell[c]{ChatGLM2, RWKV,\\LLaMA2} & Softmax & \red{$\times$} & \red{$\times$} & Recommendation & Click Prediction &1& \href{https://github.com/Xuan-ZW/LKPNR}{link} \\
      & GRID~\cite{ni2023grid} & GAT & INSTRUCTOR & Decoder & \red{$\times$} & \red{$\times$} & Robotics & Robot Task Planning & 2&\href{https://jackyzengl.github.io/GRID.github.io/}{link} \\
      & ENG~\cite{yu2023empower} & GCN,GAT & ChatGPT & GNN & \red{$\times$} & \lightgreen{$\checkmark$} & Citation & Node & - \\
      & LLM4Mo~\cite{qian2023can} & - & ChatGPT & PLM & \red{$\times$} & \lightgreen{$\checkmark$} & Molecular & Molecular Property Prediction & 3&\href{https://github.com/ChnQ/LLM4Mol}{link} \\
      & GPT-MolBERTa~\cite{balaji2023gptmolberta} & - & ChatGPT & PLM & \red{$\times$} & \lightgreen{$\checkmark$} & Molecular & Molecular Property Prediction &9& - \\
      
    \midrule
    \multicolumn{1}{c}{\multirow{25}[2]{*}{\rotatebox{90}{Predictor}}} 
      & GPT4Graph~\cite{guo2023gpt4graph} & - & text-davinci-003 & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & - & Structure,Graph,Node,KGQA &4 & \href{https://anonymous.4open. science/r/GPT4Graph}{link} \\
      & GraphText~\cite{zhao2023graphtext} & - & ChatGPT, LLaMA2-7B & LLM & \lightgreen{$\checkmark$} & \lightgreen{$\checkmark$} & Citation, Web & Node &7 & - \\
      & NLGraph~\cite{wang2023can} & - & ChatGPT, GPT-4, etc. & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & - & Structure &3 & \href{https://github.com/Arthur-Heng/NLGraph}{link} \\
      & InstructGLM~\cite{ye2023natural} & - & Flan T5, LLaMA & LLM & \lightgreen{$\checkmark$} & \lightgreen{$\checkmark$} & Citation & Node &3& \href{https://github.com/Graphlet-AI/llm-graph-ai}{link} \\
      & LLMtoGraph~\cite{liu2023evaluating} & - & \makecell[c]{ChatGPT, GPT-4,\\Vicuna-13B, etc.} & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & - & Structure &-& \href{https://github.com/Ayame1006/LLMtoGraph}{link} \\
      & Graph Agent~\cite{wang2023graph} & - & \makecell[c]{GPT-4,\\embedding-ada-002} & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & Citation, Bioinformatics & Node, Edge &2 & - \\
      & LLM-Prop~\cite{rubungo2023llmprop} & - & T5 & LLM & \lightgreen{$\checkmark$} & \red{$\times$} & materials science & Crystal Property Prediction &-& \href{https://github.com/vertaix/LLM-Prop}{link} \\
      & GLRec~\cite{wu2023exploring} & - & BELLE-LLaMA-7B & LLM & \lightgreen{$\checkmark$} & \lightgreen{$\checkmark$} & Recommendation & Recommendation &1& - \\
      & ReLM~\cite{shi2023relm} & TAG,GCN & GPT-3.5, Vicuna & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & Chemistry & Chemical Reaction Prediction & 5 & \href{https://github.com/syr-cn/ReLM}{link} \\
      & Chen et al.~\cite{chen2023exploring} & - & ChatGPT & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & Citation, E-commerce & Node &5& \href{https://github.com/CurryTang/Graph-LLM}{link} \\
      & Hu et al.~\cite{hu2023text} &   & ChatGPT,GPT-4 & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & Citation,KG & Node, Edge &5 & - \\
      & Huang et al.~\cite{huang2023can} & - & ChatGPT & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & Citation, E-commerce & Node &5 & \href{https://github.com/TRAIS-Lab/LLM-Structured-Data}{link} \\
      & Fatemi et al.~\cite{fatemi2023talk} &   & PaLM2 XXS, PaLM 62B & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & - & Structure & - & -\\

      & DrugChat~\cite{liang2023drugchat} & GAT, etc. & Vicuna-13B & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & Drug & QA &-& \href{https://github.com/UCSD-AI4H/drugchat}{link} \\
      & KoPA~\cite{zhang2023making} & RotateE & Alpaca-7B & LLM & \lightgreen{$\checkmark$} & \lightgreen{$\checkmark$} & Knowledge Graph & Knowledge Graph Completion &3& \href{https://github.com/zjukg/KoPA }{link} \\
      & GraphGPT~\cite{tang2023graphgpt} & Graph Transformer & Vicuna-7B & LLM & \lightgreen{$\checkmark$} & \lightgreen{$\checkmark$} & Citation & Node & 3& \href{https://graphgpt.github.io/c}{link} \\
      & GraphLLM~\cite{chai2023graphllm} & Graph Transformer & LLaMA2 & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & - & Structure &4& \href{https://github.com/mistyreed63849/Graph-LLM}{link} \\
      & GNP~\cite{tian2023graph} & GAT & Flan T5 & LLM & \lightgreen{$\checkmark$} & \lightgreen{$\checkmark$} & KG & KGQA &4& - \\
      & GIMLET~\cite{zhao2023gimlet} & - & T5 & LLM & \lightgreen{$\checkmark$} & \lightgreen{$\checkmark$} & Molecular & Molecular Property Prediction &14& \href{https://github.com/zhao-ht/GIMLET}{link} \\
      & GIT-Mol~\cite{liu2023gitmol} & GIN & MolT5 & LLM & \lightgreen{$\checkmark$} & \lightgreen{$\checkmark$} & Molecular & Molecular Generation, etc. &6 & - \\
      & BioMedGPT~\cite{luo2023biomedgpt} & GIN & LLaMA2-7B-Chat & LLM & \lightgreen{$\checkmark$} & \lightgreen{$\checkmark$} & Biomedical & QA & 3 & \href{https://github.com/PharMolix/OpenBioMed}{link} \\
      & ProteinChat~\cite{guo2023proteinchat} & GVP-GNN & Vicuna-13B & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & Protein & QA & 1 & \href{https://github.com/UCSD-AI4H/proteinchat}{link} \\
      & MolReGPT~\cite{li2023empowering} & - & ChatGPT & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & Molecular & molecule-caption translation & 1 & \href{https://github.com/phenixace/MolReGPT}{link} \\
      & DGTL~\cite{qin2023disentangled} & Disentangled GNN & LLaMA-2-13B-chat & LLM & \red{$\times$} & \lightgreen{$\checkmark$} & Citation, E-commerce & Node &3& - \\
      
    \midrule
    \multicolumn{1}{c}{\multirow{7}[2]{*}{\rotatebox{90}{Agent}}} 
      & Graph-ToolFormer~\cite{zhang2023graph} & - & GPTJ, LLaMA & Tool & \lightgreen{$\checkmark$} & \lightgreen{$\checkmark$} & - & Graph &15& \href{https://github.com/jwzhanggy/Graph_Toolformer}{link} \\
      & GPT4GNAS~\cite{wang2023graph(a)} & GCN, GIN, etc. & GPT-4 & GNN & \red{$\times$} & \lightgreen{$\checkmark$} & Citation & Node & -& - \\
      & Auto2Graph~\cite{wei2023unleashing} & GCN,SAGE, etc. & Not Mention & GNN & \red{$\times$} & \lightgreen{$\checkmark$} & - & Graph,Node &8 & - \\
      & SayPlan~\cite{rana2023sayplan} & - & GPT4 & Tool & \red{$\times$} & \lightgreen{$\checkmark$} & Robotics & Robot Task Planning & -&\href{https://sayplan.github.io/}{link} \\
      & SayNav~\cite{rajvanshi2023saynav} & - & ChatGPT, GPT4 & Tool & \red{$\times$} & \lightgreen{$\checkmark$} & Robotics & Robot Task Planning &- & - \\
      & Dai et al.~\cite{dai2023optimal} & - & GPT4 & Tool & \red{$\times$} & \lightgreen{$\checkmark$} & Robotics & Robot Task Planning &- & - \\
      & Think\_Net\_Prompt~\cite{zhen2023robot} & - & GPT3.5,GPT4 & Tool & \red{$\times$} & \lightgreen{$\checkmark$} & Robotics & Robot Task Planning &-& \href{https://github.com/NOMIzy/Think_Net_Prompt}{link} \\
      
    % \midrule
    % \multicolumn{1}{l}{Others} 
    %   & TF-Dcon & - & ChatGPT & LM & \red{$\times$} & \lightgreen{$\checkmark$} & Recommendation & Recommendation & - \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:llm-enhanced graph}%
\end{table*}%
